Exploring Event Camera-based Odometry for Planetary Robots

Due to their resilience to motion blur and high robustness in low-light and high dynamic range conditions, event cameras are poised to become enabling sensors for vision-based exploration on future Mars helicopter missions. However, existing event-based visual-inertial odometry (VIO) algorithms either suffer from high tracking errors or are brittle, since they cannot cope with significant depth uncertainties caused by an unforeseen loss of tracking or other effects. In this work, we introduce EKLT-VIO, which addresses both limitations by combining a state-of-the-art event-based frontend with a filter-based backend. This makes it both accurate and robust to uncertainties, outperforming event- and frame-based VIO algorithms on challenging benchmarks by 32%. In addition, we demonstrate accurate performance in hover-like conditions (outperforming existing event-based methods) as well as high robustness in newly collected Mars-like and high-dynamic-range sequences, where existing frame-based methods fail. In doing so, we show that event-based VIO is the way forward for vision-based exploration on Mars.

==> figure_computation_pie_charts.tex <==
\begin{figure*}[t]
\vspace{4ex}
\centering
\begin{tabular}{ccc}
\includegraphics[trim=0 0 0 0,clip,height=0.22\linewidth]{figures/rt_factor_poster_6dof_cropped.pdf}&
\includegraphics[height=0.22\linewidth]{figures/rtf_rtfpf_vs_event_rate_poster_translation.pdf}&
\includegraphics[trim=0 -15mm 0 0,clip, height=0.22\linewidth]{figures/computational_pie_plot_eklt.pdf}\\
(a) Realtime factor&
(b) Realtime factor vs. Event rate&
(c) Computational pie chart
\end{tabular}
\caption{\rev{Real-time factor (RTF) (a) for EKLT-VIO (orange), HASTE-VIO (green) and KLT-VIO (blue) on \emph{Poster 6DOF}. The RTF per tracked feature (b) increases with the event rate. \revtwo{Our method can process 89'000 events per second when tracking 45 features. As seen in (c), EKLT-VIO spends most of its computation time tracking features.}}}
\label{fig:rt_factor}
\end{figure*}

\iffalse
\begin{figure}
\centering
\begin{tabular}{cc}
\includegraphics[height=0.27\linewidth]{figures/computational_pie_plot_eklt.pdf}&
\includegraphics[height=0.27\linewidth]{figures/computational_pie_plot_xvio.pdf}\\
(a) EKLT-VIO (ours)&
(b) KLT-VIO
\end{tabular}
\caption{\rev{Relative computation time spent by EKLT-VIO (a) and KLT-VIO~\cite{delaune2021xvio} (b). The main bottleneck in EKLT-VIO is the feature tracker. By contrast, KLT-VIO spends most of its time in the backend.}}
\label{fig:pies}
\end{figure}
\fi


==> figure_mars_simulation_tracking.tex <==
\begin{figure*}[t]
\centering
\begin{tabular}{cc}
    \includegraphics[height=0.2\linewidth]{figures/mars-environment.jpg}&
    \includegraphics[height=0.2\linewidth]{figures/mellon.pdf}\\
(a) Virtual Mars environment&    (b) Melon trajectory 
\end{tabular}
%\begin{subfigure}{.3\linewidth}
% \centering
%    \centering
%    \includegraphics[height=1.2in]{figures/feature_tracking_vertical_circle_slow.pdf}
%    \caption{Feature tracking comparison}
%    \label{fig:feature-tracking}
%\end{subfigure}
\caption{Overview of the synthetic Mars-like dataset used in this work. We use the ``Mars Landscape" environment from Unreal Engine (a). We simulate aggressive trajectories, including the melon trajectory (b), borrowed from \cite{Bauersfeld21RSS}.}\label{fig:preview_mars_sim}
\end{figure*}

==> figure_qualitative_frontend_comparison.tex <==

\begin{figure*}[t]
\centering
\begin{tabular}{ccc}
\centering
  \includegraphics[height=.2\linewidth]{figures/capture_eklt.png}&
  \includegraphics[height=.2\linewidth]{figures/capture_haste.png}&
  \includegraphics[height=.2\linewidth]{figures/capture_xvio.png}\\
  (a) EKLT frontend&(b) HASTE frontend&(c) KLT frontend
\end{tabular}

% \begin{subfigure}{.33\linewidth}
%   \includegraphics[width=\linewidth]{figures/rpe_errors_shapes_6dof.pdf}
%     \caption{Shapes 6DOF}
%     \label{fig:rpg-error-hdr-poster}
% \end{subfigure}
\caption{Qualitative frontend performance comparison on poster rotation sequence: The proposed event-based methods (a,b) manage to maintain SLAM feature tracks (in green) also under motion-blur and low light condition, where the frame-based frontend (c) fails. Maintaining a stable number of SLAM features is essential for robust pose estimation.}
\label{fig:capture-poster-rotation}

\end{figure*}

==> figure_rpe_boxplots_davis_data.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}{.5\linewidth}
  \includegraphics[width=\linewidth]{figures/rpe_errors_shapes_6dof.pdf}
    \caption{Boxes 6DOF}
    \label{fig:rpg-error-shapes-6dof}
\end{subfigure}%
% \hspace{1cm}%
\begin{subfigure}{.5\linewidth}
  \includegraphics[width=\linewidth]{figures/rpg_errors_hdr_poster.pdf}
    \caption{HDR Poster}
    \label{fig:rpg-error-hdr-poster}
\end{subfigure}
\caption{Relative pose errors from pairs at different distances on RPG DAVIS datasets. EKLT-VIO significantly outperforms Ultimate SLAM in relative pose accuracy on most sequences.}
\label{fig:rpe-error-davis-data}

\end{figure*}

==> previous_intro.tex <==



For mobile robots, ego-motion estimation is one of the most crucial tasks enabling control and autonomous navigation with wide-spread applications from space exploration to household cleaning robots.
There exist well established algorithms, such as \cite{li2013msckfslam} and \cite{forster2016manifold}, processing visual-inertial information obtaining robust state estimation.
Due to the known limitations of conventional frame-based cameras such as motion blur and low dynamic range, these are however inherently limited in their range of feasible applications.
For instance, entering and exploring a cave poses challenges due to abrupt brightness changes and low-lighting condition.

Progress has been made exploiting a novel type of vision sensor, namely event-based cameras \cite{gallego2019event}.
Instead of measuring absolute pixel brightness using a global exposure time, each pixel independently detects logarithmic brightness changes triggering events with positive or negative polarity at a high temporal resolution.
This leads to resilience to motion blur and high dynamic range (120dB vs 60dB of standard frame-based cameras).
Current state of the art visual inertial odometry approaches exploit both frames and events, as in \cite{vidal2018ultimate}.

Visual inertial odometry pipelines are typically split into front- and backend. The frontend is detecting and tracking features in the image plane and the backend is taking care of pose estimation and eventual loop-closures.
Main approaches can be divided into filter-based and optimization based methods.
Optimization based approaches such as \cite{vidal2018ultimate} usually use so-called keyframes where features get triangulated and the pose estimate optimized to fit multiple observations in the past.
Filter-based approaches exploit visual measurement models for an Extended Kalman Filter, This usually requires extending the state, either by triangulated feature positions, known as SLAM features, or by a sliding window of history of poses to indirectly exploit feature tracks, known as MSCKF.

In this work we leverage the low latency and high temporal resolution of event cameras for filter-based visual intertial odometry.
They confer the following advantages on our algorithm:

\begin{enumerate}
    \item increased filter stability through high update rates
    \item robustness to high dynamic range and motion blur and
    \item high frequency state update for fine-grained localization
\end{enumerate}

\subsection{Contributions}

Our contributions are three-fold:

\begin{itemize}
    \item Integration of two event-based feature trackers in EKF backend
    \begin{itemize}
        \item Extensive accuracy and realtime performance comparisons of Ultimate SLAM \cite{vidal2018ultimate}, frame-based xVIO \cite{delaune2020xvio} and our proposed pipelines with event-trackers 
    \end{itemize}
    \item First insights on the link between feature-tracking error and localization error
    % \item First feature tracking error comparisons between frame-based KLT, EKLT and HASTE in simulation
    % \begin{itemize}
    %     \item quantifying performance gap between KLT and EKLT in \cite{gehrig2020eklt}
    %     \item first comparison between SOTA event trackers
    % \end{itemize}
    \item We release a new texture-rich, photo-realistic synthetic dataset for planetary exploration
\end{itemize}



==> sim.tex <==
\subsection{Simulation}
\label{sub:sim}
\textbf{Simulated Dataset} We generate a new synthetic Mars Dataset, targeting our use-case of future Mars helicopter missions. We use three real-world drone trajectories of increasing difficulty, \rev{affected by aerodynamic effects}, and based on filtered OptiTrack measurements that were originally used in~\cite{Bauersfeld21RSS}:
%To do this, we use three real-world drone trajectories based on filtered OptiTrack measurements, which were originally used in~\cite{Bauersfeld21RSS}. Three different real-world drone trajectories with increasing difficulty were evaluated. 
\begin{itemize}
\item \textit{Mars vertical circle (slow)} features a circle of 2.5 m radius flown vertically with a downward-facing camera at less than 2.4 m/s.
\item \textit{Mars horizontal circle (fast)} flies a horizontal circle of 4.5m radius flown at 7.2m/s peak velocity.
\item \textit{Mars \rev{ellipsoid} trajectory (very fast)} has a 4.5m, 3m and 2m radius in x, y and z direction respectively, with a peak velocity of 12.4m/s, and is illustrated in Fig.~\ref{fig:preview_mars_sim} (b). 
\end{itemize}

We deploy these trajectories in the event camera simulator, ESIM~\cite{rebecq2018esim}, with the Unreal Engine 4.26 as the rendering backend, running the ``Mars Landscape" environment (Fig. \ref{fig:preview_mars_sim} (a)). \rev{This environment simulates the visual appearance on Mars. It currently does not support dust simulation, which would be future work.} The dataset contains events, frames and noisy IMU measurements. Since USLAM is sensitive to initial IMU biases, we append an initial bootstrapping part with translatory motion, which guarantees IMU bias convergence.  \rev{We denote this method by USLAM*.} All other methods are initialized with pose ground-truth at 10s.

%\davide{What are the radii of the circles? Please be accuraate in describing the setups.}
\textbf{Results} The tracking performance results are reported in Tab.~\ref{tab:sim-pose}.
While frame-based KLT-VIO outperforms the other methods on the slow sequence with a mean position error (MPE) of 0.73\% , event-based approaches show superior performance on the faster sequences. Indeed, EKLT-VIO outperforms all other methods with an MPE of 2.43\%. The runner-up is USLAM$^*$ which features a 19\% higher average MPE. These results show that, especially in high-speed scenarios, event-cameras are necessary, since KLT-VIO diverges on the Mars \rev{ellipsoid} trajectory. Moreover, our method maintains the lowest tracking error at high-speed, outperforming all other frame- or event-based methods.%\davide{But EKLT-VIO (ours) gets 9.77\% MPE vs. 2.24\% of Ultimate SLAM. Elaborate why.}
%To further demonstrate understand the importance of event-based frontends we perform a feature tracking analysis, based on the \footnote{\url{https://github.com/uzh-rpg/rpg_feature_tracking_analysis}}{feature tracking toolbox} used in~\cite{gehrig2020eklt}, which we show in Fig.\ref{fig:feature-tracking}. 
%Here EKLT-VIO shows shows the most accurate and consistent feature tracking performance. This higher accuracy translates in a more consistent and robust tracking performance. %We further evaluate all feature tracks with respect to ground truth in \cref{fig:feature-tracking}, showing the average of all tracking errors over the whole sequences, by aligning their start time.
% \begin{itemize}
%     \item some results like in \cref{fig:feature-tracking}
% \end{itemize}
%\input{figure_qualitative_frontend_comparison}

==> table_rpg_davis_rotation_absolute.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[t]
% \resizebox{\textwidth}{!}{%
\centering
\begin{tabular}{@{}lcccccccc@{}}
\toprule
Dataset & \multicolumn{2}{c}{USLAM~\cite{Rosinol18ral}} &\multicolumn{2}{c}{KLT-VIO~\cite{delaune2021xvio}} & \multicolumn{2}{c}{HASTE-VIO}  & \multicolumn{2}{c}{EKLT-VIO (\textbf{ours})}\\ \midrule
& MPE & MYE & MPE & MYE & MPE & MYE & MPE & MYE \\ \midrule
Dynamic Rotation & \multicolumn{2}{c}{\multirow{4}{*}{\textit{unfeasible}}}                                                                                                                                        & 1.73m                                                                        & \textbf{1.7°}                                                                   & \textbf{1.06m}                                                               & \multicolumn{1}{c|}{30.8°}& 1.31m                                                                        & 20.2°                                                                                                                                                        \\
Boxes Rotation   & \multicolumn{2}{c}{}                                                                                                    & \multicolumn{2}{c}{\textit{diverging}}                                                                                                                        & 1.90m                                                                       & \multicolumn{1}{c|}{\textbf{15.5°}} & \textbf{0.81m}                                                               & 16.0°\\
Poster Rotation  & \multicolumn{2}{c}{}                                                                                                                                        & \multicolumn{2}{c}{\textit{diverging}}                                                                                                                        & 3.00m                                                                        & \multicolumn{1}{c|}{\textbf{72.0°}}                                                                   & \textbf{1.09m}                                                               & \textbf{72.0°}                                                                   \\ 
Shapes Rotation  & \multicolumn{2}{c}{}                                                                                                                                        & \multicolumn{2}{c}{\textit{diverging}}                                                                                                                        & \multicolumn{2}{c|}{\textit{diverging}}& \textbf{0.24m}                                                               & \textbf{1.6°}                                                                                                                                                                                           \\\bottomrule
\end{tabular}%
% }
\caption{Pose estimation accuracy in terms of mean position error (MPE) in meters and mean yaw error (MYE) in degrees on rotation-only sequences. The normalization on the traveled distance is obsolete on rotation only sequences, since it is close to zero.}
\label{tab:rpg-davis-rotation}
\vspace{-2ex}
\end{table*}

==> table_sim_pose_accuracy.tex <==
\begin{figure*}[t]
\centering
\begin{tabular}{cc}
    \includegraphics[height=0.2\linewidth]{figures/mars-environment.jpg}&
    \includegraphics[height=0.2\linewidth]{figures/mellon.pdf}\\
(a) Virtual Mars environment&    (b) \rev{Ellipsoid} trajectory 
\end{tabular}
%\begin{subfigure}{.3\linewidth}
% \centering
%    \centering
%    \includegraphics[height=1.2in]{figures/feature_tracking_vertical_circle_slow.pdf}
%    \caption{Feature tracking comparison}
%    \label{fig:feature-tracking}
%\end{subfigure}
\caption{Overview of the synthetic Mars-like dataset used in this work. We use the ``Mars Landscape" environment from Unreal Engine (a). We simulate aggressive trajectories, including the \rev{Ellipsoid} trajectory (b), borrowed from \cite{Bauersfeld21RSS}.}\label{fig:preview_mars_sim}
\end{figure*}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\iffalse
\begin{table*}[t]
\centering
\begin{tabular}{@{}lcccccccc@{}}
\toprule
Dataset & \multicolumn{2}{c}{USLAM~\cite{Rosinol18ral}} & \multicolumn{2}{c}{KLT-VIO~\cite{delaune2021xvio}} & \multicolumn{2}{c}{EKLT-VIO (\textbf{ours})} & \multicolumn{2}{c}{HASTE-VIO (\textbf{ours}) } \\ \midrule
 & MPE  & MYE & MPE   & MYE  & MPE   & MYE  & MPE   & MYE  \\ \midrule
Mars vertical circle (slow) & 8.93 & \textbf{1.7} & \textbf{0.73} & \multicolumn{1}{c|}{0.50} & 2.32 & 2.84 & 2.53 & 1.21 \\
Mars horizontal circle (fast)  & 7.71 & 0.11 & 4.12 & \multicolumn{1}{c|}{0.04} & \textbf{1.89} & \textbf{0.03} & 3.98 & 0.07 \\
Mars horizontal circle (very fast) & \textbf{2.24} & \textbf{0.01} & 48.69 & \multicolumn{1}{c|}{0.22} & 9.77 & 0.03 & 5.93 & 0.01 \\ \bottomrule
\\
\textbf{Average} & xx & xx & xx & xx & xx & xx & xx & xx\\\bottomrule
\end{tabular}
\caption{Pose estimate accuracy comparison in simulated Mars environment, in terms of mean position error (MPE) in \% and mean yaw error (MYE) in deg/m.}
\label{tab:sim-pose}
\end{table*}
\fi

\begin{table*}[t]
\centering
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
Dataset & \multicolumn{2}{c}{\lightgray{USLAM*~\cite{Rosinol18ral}}} &\multicolumn{2}{c}{USLAM~\cite{Rosinol18ral}} & \multicolumn{2}{c}{KLT-VIO~\cite{delaune2021xvio}} & \multicolumn{2}{c}{HASTE-VIO} & \multicolumn{2}{c}{EKLT-VIO (\textbf{ours})} \\ \midrule
&\lightgray{MPE} & \lightgray{MYE} & MPE  & MYE & MPE   & MYE&  MPE   & MYE&  MPE   & MYE  \\ \midrule
Mars vertical circle (slow)& \lightgray{5.76}& \lightgray{1.80}& 59.58 & 2.21 & \textbf{0.73} & \textbf{0.50}& 1.44 & \multicolumn{1}{c|}{1.28} & 2.11 & 1.89\\
Mars horizontal circle (fast) &\lightgray{1.43} & \lightgray{0.02} & 1.58  & 0.03  & 4.12 & 0.04 & 98.90 & \multicolumn{1}{c|}{0.47}& \textbf{1.23} & \textbf{0.01} \\
Mars \rev{ellipsoid} trajectory (very fast) &\lightgray{1.79}&\lightgray{0.08}& 108.73 & 0.08  & 190.6 & 0.03 & 32.14 & \multicolumn{1}{c|}{0.17} & \textbf{3.95} & \textbf{0.02}\\ \bottomrule
\multicolumn{11}{l}{\rev{*per-sequence hyperparameter tuning and correct IMU bias intialization}}\\\bottomrule
%\\
%\textbf{Average} &\lightgray{2.99}& \lightgray{0.63}&56.64  & 0.77  & 65.15 & \textbf{0.19} & \textbf{2.43} & 0.64 & 44.16 & 0.64\\\bottomrule
\end{tabular}
\caption{Pose estimate comparison on our simulated Mars environment. Accuracy is reported in terms of mean position error (MPE) in \% and mean yaw error (MYE) in deg/m. Our method EKLT-VIO outperforms state-of-the-art frame-based and event-based methods~\cite{Rosinol18ral,delaune2021xvio}. Both USLAM and KLT-VIO diverge on the challenging, high-speed Mars mellon trajectory. For this reason, we first initialize USLAM with a slow 10 second bootstrapping sequence before executing the trajectory, shown \rev{in gray with a (*)}. Despite this help, USLAM still has a 19\% higher average MPE than EKLT-VIO.}
\label{tab:sim-pose}
\end{table*}
